OxyGen: Unified KV Cache Management for VLA Inference under Multi-Task Parallelism

Embodied AI agents increasingly require parallel execution of multiple tasks, such as manipulation, conversation, and memory construction, from shared observations under distinct time constraints. Recent Mixture-of-Transformers (MoT) Vision-Language-Action Models (VLAs) support such heterogeneous outputs, yet existing inference systems incur redundant computation and resource contention when serving concurrent tasks on-device. We identify isolated KV cache management as the root cause. To address this, we propose unified KV cache management, an inference design that treats the KV cache as a first-class shared resource across tasks and control cycles. This abstraction enables two key optimizations: cross-task KV sharing eliminates redundant prefill of shared observations, while cross-frame continuous batching batches unfinished language requests from different frames and advances them within a per-frame decoding budget. We implement this design in OxyGen and evaluate $\pi_{0.5}$ on NVIDIA GeForce RTX 4090 and Jetson AGX Thor. OxyGen achieves up to 3.7$\times$ speedup over isolated execution, delivering over 200 tokens/s language throughput and 70 Hz action frequency simultaneously on RTX 4090. We also validate the design on Xiaomi-Robotics-0 and StarVLA across different backbones and expert configurations. We further demonstrate the inference gains on a humanoid robot with on-board Jetson AGX Thor.

==> tex/air_frontmatter.tex <==
\makeatletter
\newcommand{\AIRpdfauthors}{}
\newcommand{\AIRcollectauthors}{%
  \gdef\AIRpdfauthors{}%
  \begingroup
  \def\PaperAuthor##1##2##3{%
    \ifx\AIRpdfauthors\@empty\else\g@addto@macro\AIRpdfauthors{, }\fi
    \g@addto@macro\AIRpdfauthors{##1}}%
  \PaperAuthors
  \endgroup}
\makeatother
\newcommand{\AIRrenderauthors}[1]{%
  \def\AIRauthorseparator{}%
  \def\PaperAuthor##1##2##3{\AIRauthorseparator##1$^{##2##3}$\def\AIRauthorseparator{\space#1}}%
  \PaperAuthors}
\newcommand{\AIRrenderlinks}[1]{%
  \def\AIRlinkseparator{}%
  \def\PaperLink##1##2{\AIRlinkseparator\textbf{##1:} \url{##2}\xspace\def\AIRlinkseparator{#1}}%
  \PaperLinks}
\newcommand{\AIRpdfauthorblock}{%
  \AIRrenderauthors{\quad}\\
  \medskip
  {\AIRaffiliationfont
    \def\PaperAffiliation##1##2##3{$^{##1}$##2##3}%
    \PaperAffiliations
    \def\PaperNote##1##2{$^{##1}$##2\\}%
    \PaperNotes}%
  \medskip
  {\AIRprojectfont\AIRrenderlinks{\\}}}
\makeatletter
\newcommand{\AIRcameraauthorblock}{}
\newcommand{\AIRsetupcameraauthors}{%
  \AIRcollectauthors
  \gdef\AIRcameraauthorblock{}%
  \begingroup
    \def\PaperAuthor##1##2##3{%
      \ifx\AIRcameraauthorblock\@empty\else
        \g@addto@macro\AIRcameraauthorblock{ \enspace }\fi
      \g@addto@macro\AIRcameraauthorblock{##1$^{##2##3}$}}%
    \PaperAuthors
    \g@addto@macro\AIRcameraauthorblock{ \\ }%
    \def\PaperAffiliation##1##2##3{%
      \g@addto@macro\AIRcameraauthorblock{$^{##1}$##2 \\ }}%
    \PaperAffiliations
    \def\PaperNote##1##2{%
      \g@addto@macro\AIRcameraauthorblock{$^{##1}$##2 \\ }}%
    \PaperNotes
    \def\AIRlinkseparator{}%
    \def\PaperLink##1##2{%
      \ifx\AIRlinkseparator\@empty\else
        \g@addto@macro\AIRcameraauthorblock{ \\ }\fi
      \g@addto@macro\AIRcameraauthorblock{\textbf{##1:} \url{##2}\xspace}%
      \def\AIRlinkseparator{used}}%
    \PaperLinks
  \endgroup
  \author{\AIRcameraauthorblock}}
\makeatother
\newcommand{\AIRsetupauthors}{%
  \AIRcollectauthors
  \iflatexml
    \def\PaperAuthor##1##2##3{\author[##2]{##1\textsuperscript{\ensuremath{##3}}}}%
    \PaperAuthors
    \def\PaperAffiliation##1##2##3{\affil[##1]{##2}}%
    \PaperAffiliations
  \else
    \AIRauthorblock{\AIRpdfauthorblock}%
  \fi}

